Orienting supersingular isogeny graphs

We introduce a category of $\mathcal{O}$-orientedsupersingularellipticcurves and derive properties of the associated oriented and nonoriented $\ell$-isogeny supersingular isogeny graphs. As an application we introduce an oriented super-singular isogeny Diffie-Hellman protocol (OSIDH), analogous to the supersingular isogeny Diffie-Hellman (SIDH) protocol and generalizing the commutative supersingular isogeny Diffie-Hellman (CSIDH) protocol.

==> SECTIONS/HardProblems.tex <==
\section{Hard Problems}

\begin{problem}[Endomorphism ring problem]\label{problem:endomorphismring}
Given a supersingular elliptic curve $E/\FF_{p^2}$ and $\pi=\left[ p\right]$, determine
\begin{description}
\item[1.] $\End(E)$ as an abstract ring.
\item[2.] An explicit endomorphism $\phi\in\End(E)\setminus\ZZ$.
\item[3.] An explicit basis $\mathfrak{B}^0$ for $\End^0(E)$ over $\QQ$.
\item[4.] An explicit basis $\mathfrak{B}$ for $\End(E)$ over $\ZZ$.
\end{description}
\end{problem}

\begin{problem}[Endomorphism ring transfer problem]\label{problem:endomorphismringtransfer}
	Given an isogeny chain
	\[
	E_0\longrightarrow E_1\longrightarrow\ldots\longrightarrow E_n
	\]
	and $\End(E_0)$, determine $\End(E_n)$.
\end{problem}

\begin{problem}\label{problem:endomorphismgenerator}
	Given a supersingular elliptic curve $E/\FF_{p^2}$, $\pi=\left[p\right]$, an imaginary quadratic order $\OO$ admitting an embedding in $\End(E)$ and a collection of compatible $(\OO,\mathfrak{q}^n)$-orientations of $E$ for $(\mathfrak{q},n)\in S$, determine 
	\begin{description}
		\item[1.] An explicit endomorphism $\phi\in\OO\subseteq \End(E)$
		\item[2.] A generator $\phi$ of $\OO\subseteq \End(E)$
	\end{description}
\end{problem}

Suppose $S=\{(\mathfrak{q},n) \}=\{(\mathfrak{q}_1,n_1),\ldots,(\mathfrak{q}_t,n_t)\}$ where $\mathfrak{q}_1,\mathfrak{q}_t$ are pairwise distinct primes such that 
\begin{align}\label{Injectivemap:primes}
[0,\ldots,n_1]\times\ldots\times[0,\ldots,n_t]\longrightarrow&~\Cl(\OO)\\
(e_1,\ldots,e_t)\longrightarrow&~[\mathfrak{q}_1^{e_1}\cdot\ldots\cdot\mathfrak{q}_t^{e_t}]\nonumber
\end{align}
is injective.
Then, Problem \ref{problem:endomorphismgenerator} should remain difficult.

We can reformulate this in a way that allows $(\bar{\mathfrak{q}}_i,n_i)\in S$: For instance, assume that $S$ is closed under $(\mathfrak{q}_i,n_i)\to(\bar{\mathfrak{q}}_i,n_i)$ and replace (\ref{Injectivemap:primes}) with 
\begin{align}\label{Injectivemap:primes_bis}
[-n_1,\ldots,n_1]\times\ldots\times[-n_t,\ldots,n_t]\longrightarrow&~\Cl(\OO)\\
(e_1,\ldots,e_t)\longrightarrow&~[\mathfrak{q}_1^{e_1}\cdot\ldots\cdot\mathfrak{q}_t^{e_t}]\nonumber
\end{align}
injective.
\begin{remark}
For a negative integer $e_i<0$, the power $\mathfrak{q}_i^{e_i}$ corresponds to $\bar{\mathfrak{q}}_i^{-e_i}$.
\end{remark}
